Analyzing mechanisms and microscopic reversibility of self-assembly

We use computer simulations to investigate self-assembly in a system of model chaperonin proteins, and in an Ising lattice gas. We discuss the mechanisms responsible for rapid and efficient assembly in these systems, and we use measurements of dynamical activity and assembly progress to compare their propensities for kinetic trapping. We use the analytic solution of a simple minimal model to illustrate the key features associated with such trapping, paying particular attention to the number of ways that particles can misbind. We discuss the relevance of our results for the design and control of self-assembly in general.

==> PaxHeader/grant_traffic_revised_jcp.tex <==
18 gid=1552001941
18 uid=1632763755
20 ctime=1319111036
20 atime=1323344432
38 LIBARCHIVE.creationtime=1319111011
24 SCHILY.dev=234881026
23 SCHILY.ino=10901864
18 SCHILY.nlink=1

